TrustUQA: A Trustful Framework for Unified Structured Data Question Answering

Natural language question answering (QA) over structured data sources such as tables and knowledge graphs have been widely investigated, especially with Large Language Models (LLMs) in recent years. The main solutions include question to formal query parsing and retrieval-based answer generation. However, current methods of the former often suffer from weak generalization, failing to dealing with multi-types of sources, while the later is limited in trustfulness. In this paper, we propose TrustUQA, a trustful QA framework that can simultaneously support multiple types of structured data in a unified way. To this end, it adopts an LLM-friendly and unified knowledge representation method called Condition Graph(CG), and uses an LLM and demonstration-based two-level method for CG querying. For enhancement, it is also equipped with dynamic demonstration retrieval. We have evaluated TrustUQA with 5 benchmarks covering 3 types of structured data. It outperforms 2 existing unified structured data QA methods. In comparison with the baselines that are specific to one data type, it achieves state-of-the-art on 2 of the datasets. Further more, we have demonstrated the potential of our method for more general QA tasks, QA over mixed structured data and QA across structured data. The code is available at https://github.com/zjukg/TrustUQA.

==> tables/ErrorType.tex <==
\begin{table*}[]
\centering
\renewcommand{\arraystretch}{1.0}
\resizebox{1.\textwidth}{!}{
\begin{tabular}{@{}l|l|l|l@{}}
\toprule
\multicolumn{1}{c|}{\textbf{Error Type}} &
  \multicolumn{1}{c|}{\textbf{Question}} &
  \multicolumn{1}{c|}{\textbf{Query}} &
  \multicolumn{1}{c}{\textbf{Analysis}} \\ \midrule
% \multirow{4}{*}{query \\generation \\errors} &
% \multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}query \\ generation   \\ errors\end{tabular}} &
\multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}\textbf{Query} \\ \textbf{generation}   \\ \textbf{error}\end{tabular}} &
  \begin{tabular}[c]{@{}l@{}} Who co-wrote films \\with [Howard Hawks] \end{tabular}&
  \begin{tabular}[c]{@{}l@{}}Step1: Find films written by Howard Hawks\\Query1: ``\textit{get\_information(relation=`written\_by',} \textbf{\textit{head\_entity}}\textit{=}\\\textit{`Howard Hawks'})"...\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Logical error. \\\textit{Howard Hawks} should be the tail entity.\end{tabular} \\
   \cline{2-4} 
 &
  \begin{tabular}[c]{@{}l@{}}Which was the first award \\that Alain Resnais received \end{tabular}&
  \begin{tabular}[c]{@{}l@{}}... Step2: Get the first time of output\_of\_query1\\Query2: ``\textit{min(set=`output\_of\_query1')}"\\ \textbf{Missing one step query for award.}\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Unclear logic in query. One step is missing.\end{tabular}\\
  \cline{2-4} 
 &
  \begin{tabular}[c]{@{}l@{}}Which year Glenn Robert Davis \\first became delegate \end{tabular}&
  \begin{tabular}[c]{@{}l@{}}Step1: Find  year Glenn that Robert Davis first became delegat\\Query1: ``\textit{get\_information(head\_entity=`Glenn Robert Davis',} \\ \textit{relation=`position held', tail\_entity=`delegate',} \\\textbf{\textit{adj=`first'}}\textit{, key=`time')}"\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Grammar error. \\adj=`first' is not designed in grammar.\end{tabular} \\
  % \cline{2-4} 
 % &
 %  \begin{tabular}[c]{@{}l@{}}What are fun things to do \\in sacramento ca? \end{tabular}&
 %  \begin{tabular}[c]{@{}l@{}}Step1: Find fun activities in Sacramento, CA\\ Query1: ``get\_information(relation=`\textbf{location.location.advantages}', \\head\_entity=`Sacramento')"\end{tabular} &
 %  \begin{tabular}[c]{@{}l@{}}Error in entity and relation generation.The relation should \\be `travel.tourist\_attraction.near\_travel\_destination'\end{tabular} \\ 
  \midrule
% \multirow{2}{*}{mapping error} &
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}\textbf{Mapping} \\ \textbf{error}\end{tabular}} &
  \begin{tabular}[c]{@{}l@{}}Name the Trofeo Fast team for \\roberto visentini \end{tabular}&
  \begin{tabular}[c]{@{}l@{}}Step1: Find the entity named Roberto Visentini\\Query1: ``\textit{get\_information(relation=`\textbf{Name}', tail\_entity=}\\\textit{`Roberto Visentini')}"\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Error in relation mapping.\\The relation should map \textit{winner} but get \textit{Name}.\end{tabular} \\
  \cline{2-4} 
 &
  \begin{tabular}[c]{@{}l@{}}Who did the Red Sox play \\against on July 8? \end{tabular}&
  \begin{tabular}[c]{@{}l@{}}Step1: Find the entity that belongs to the Red Sox team\\Query1: ``\textit{get\_information(relation=`Record', tail\_entity=}\\\textit{`\textbf{@ White Sox}'})"…\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Error in entity mapping.\\Mapping should get \textit{Red Sox} but \textit{@ White Sox}.\end{tabular} \\ \midrule
% LLM function execution error &
\begin{tabular}[c]{@{}l@{}}\textbf{LLM function} \\ \textbf{execution error}\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Did the maico team earn more \\points than the cz team? \end{tabular}&
  \begin{tabular}[c]{@{}l@{}}Information provided:...\\ Just tell me the answer in a word or phrase without spaces\\ or newlines.\\Response:\textbf{Yes}\end{tabular} &
  The answer is ``No" but given ``Yes". \\ \bottomrule

    \end{tabular}
}
\caption{Cases and analysis of different types of errors.}
\vspace{-3mm}
\label{tab:ErrorType}
\end{table*}


% \begin{table}[*]
%     \centering
%     \begin{tabular}{c|c}
%          &  \\
%          & 
%     \end{tabular}
%     \caption{Caption}
%     \label{tab:my_label}
% \end{table}

==> tables/tableQA_gpt4.tex <==
\begin{table}{}
    \centering
    % \small
\caption{Denotation accuracy of fixed-schema knowledge QA on GPT4.}
% \vspace{0.7mm}
\label{tab:tableQA_gpt4}
\begin{tabular}{@{}l|cc@{}}
\toprule
\textbf{Method}       & \textbf{WikiSQL} & \textbf{WTQ}  \\ \midrule
UniT(GPT3.5) & 85.9    & 44.2 \\
UniT(GPT4)   & 87.4 ($\uparrow 1.5$)    & 52.1 ($\uparrow 7.9$) \\ \bottomrule
\end{tabular}
\end{table}
